Action-depedent Control Variates for Policy Optimization via Stein's Identity

Policy gradient methods have achieved remarkable successes in solving challenging reinforcement learning problems. However, it still often suffers from the large variance issue on policy gradient estimation, which leads to poor sample efficiency during training. In this work, we propose a control variate method to effectively reduce variance for policy gradient methods. Motivated by the Stein's identity, our method extends the previous control variate methods used in REINFORCE and advantage actor-critic by introducing more general action-dependent baseline functions. Empirical studies show that our method significantly improves the sample efficiency of the state-of-the-art policy gradient approaches.

==> Tex/bak.tex <==


\subsection{Proximal Policy Optimization with Stein control variate derivation}

\subsubsection{Gradient w.r.t parameter of $\Sigma$}
Original vanilla policy gradient w.r.t parameter of $\Sigma$:
\begin{align*}
\nabla_{\theta_\Sigma}J = \E_{\pi(a_t|s_t)}[\nabla_{\theta_\Sigma} \log \pi(a_t|s_t)\hat A_t].
\end{align*}

Take $\hat \phi(a_t, s_t) = \nabla_{a} \log\pi(a_t| s_t)\phi(a_t, s_t)$ into Stein's identity, we have
\begin{align*}
\E_{\pi(a_t|s_t)}[\nabla_a\log \pi(a_t| s_t) \cdot \nabla_a\log \pi(a_t|s_t)\phi(a_t, s_t) + \phi(a_t, s_t)\nabla_{a,a}\log\pi(a_t|s_t) + \nabla_{a}\log \pi(a_t | s_t) \cdot\nabla_a \phi(a_t | s_t)] = 0.
\end{align*}

Note that $\nabla_{\Sigma}\log\pi(a_t| s_t)= \frac{1}{2}[\nabla_{a, a}\log \pi(a_t | s_t) +  \nabla_a\log \pi(a_t| s_t) \cdot \nabla_a\log \pi(a_t|s_t)]$, we can get
\begin{align}
\E_{\pi(a_t| s_t)}[2\nabla_{\Sigma}\log \pi(a_t| s_t) + \nabla_{a}\log \pi(a_t | s_t) \cdot\nabla_a \phi(a_t | s_t)] = 0.
\label{equ:steinsigm_1}
\end{align}

If we take $\hat \phi(a_t, s_t) = \nabla_{a}\phi(a_t,s_t)$, we can Stein's Identity as 
\begin{align} 
\E_{\pi(a_t|s_t)}[\nabla_{a}\log\pi(a_t|s_t)\cdot \nabla_{a}\phi(a_t, s_t) + \nabla_{a, a}\phi(a_t, s_t)] = 0.
\label{equ:steinsigm_2}
\end{align}

If we consider use $\int\nabla_{a, a}(\pi(a_t| s_t)\phi(a_t, s_t)) = 0$, we we can get an equation which is equivalent to 
equation \eqref{equ:steinsigm_1} plus equation \eqref{equ:steinsigm_2}:
\begin{align}
\E_{\pi(a_t| s_t)}[2\nabla_{\Sigma}\log \pi(a_t| s_t) + 2\nabla_{a}\log \pi(a_t | s_t) \cdot\nabla_a \phi(a_t | s_t) + \nabla_{a, a}\phi(a_t, s_t)] = 0. 
\end{align}

If we only consider equation \eqref{equ:steinsigm_1} and take $\hat \phi(a_t, s_t) = \frac{\partial\Sigma}{\partial\theta_{\Sigma}}\phi(a_t, s_t)$, we can get unbiased policy gradient w.r.t $\theta_{\Sigma}$:
\begin{align*}
\nabla_{\theta_{\Sigma}}J &=  \E_{\pi(a_t|s_t)}[\nabla_{\theta_\Sigma} \log \pi(a_t|s_t)(\hat A_t - \phi(a_t, s_t)) - \frac{1}{2}\nabla_{a}\log \pi(a_t|s_t)\cdot\nabla_{a}\phi(a_t, s_t)\frac{\partial \Sigma}{\partial \theta_{\Sigma}}] \\
& = \E_{\pi(a_t|s_t)}[\nabla_{\theta_\Sigma} \log \pi(a_t|s_t)(\hat A_t - \phi(a_t, s_t)) +\frac{1}{2}\nabla_{a,a}\phi(a_t,s_t)\frac{\partial\Sigma}{\partial\theta_{\Sigma}}].
\end{align*}

\subsubsection{Gradient w.r.t parameter of $\mu$}
Similarly, we have 
\begin{align}
\nabla_{\theta_\mu} J = \E_{\pi(a_t|s_t)}[\nabla_{\theta_\mu} \log \pi(a_t|s_t)(\hat{A}_t -\phi(s_t,a_t)) + \nabla_a \phi(s_t,a_t) \frac{\partial \mu}{\partial {\theta_\mu}}] 
\label{equ:steinmu_1}
\end{align}




\subsection{Relation to Q-prop}
In \citep{Gu2016QPropSP}, the authors proposed to learn the action-value function off-policy. The core idea is to use the first-order Taylor expansion of the critic as a control variate, resulting in an analytically gradient term through the critic and a Monte Carlo policy gradient term consisting of the residuals in advantage approximations. Specially, Q-prop update through the following equation, 
\begin{align}
\label{equ:qprop}
\nabla_\theta J(\theta) = \mathbb{E}_{\rho_\pi,\pi}[\nabla_\theta \log \pi_\theta(a_t|s_t) ({A}(s_t,a_t) -\bar{A}_w(s_t,a_t)] + \mathbb{E}_{\rho_\pi}[\nabla_{a}  Q_w(s_t,a)|_{a= \mu_\theta(s_t)} \nabla_\theta  \mu_\theta(s_{t})] 
\end{align}
where $\rho_\pi$ is state distribution, $Q_w(s,a)$ is critic function , ${A}(s_t,a_t)$ is advantage function, and $\bar{A}(s_t,a_t) = \bar{Q}(s_t,a_t) - \mathbb{E}_{\pi_\theta}[\bar{Q}(s_t,a_t)] = \nabla_{a}Q_w(s_t,a)|_{a= \mu_\theta(s_t)}(a_t -  \mu_\theta(s_t))$. 
For the sake of clean notation, we will drop $\rho_\pi$ when possible.

Recall our update rule for $\theta_\mu$, 
\begin{align*}
\nabla_{\theta_\mu} J = \E_{\pi(a_t|s_t)}[\nabla_{\theta_\mu} \log \pi(a_t|s_t)(\hat{A}_t -\phi(s_t,a_t)) \nabla_{\theta_\mu} \mu + \nabla_a \phi(s_t,a_t) \frac{\partial \mu}{\partial {\theta_\mu}}] 
\end{align*}
in the above equation, if we use $\phi(s_t, a_t) = \bar{A}(s_t,a_t) =\nabla_a Q(s_t,\bar{a}_t)(a_t -\bar{a}_t)$, it is exactly the same as $\theta_\mu$ update part of Q-prop.

Similarly, recall that we update $\theta_\Sigma$ by using 
\begin{align*}
\nabla_{\theta_\Sigma} J = \E_{\pi(a_t|s_t)}[\nabla_{\theta_\Sigma} \log \pi(a_t|s_t)(\hat A_t - \phi(a_t, s_t)) +\frac{1}{2}\nabla_{a,a}\phi(a_t,s_t)\frac{\partial\Sigma}{\partial\theta_{\Sigma}}],
\end{align*}
if we choose $\phi(s_t, a_t) = \bar{A}(s_t,a_t) =\nabla_a Q(s_t,\bar{a}_t)(a_t -\bar{a}_t)$ then it also reduces to $\theta_\Sigma$ update part of Q-prop.

Note that in Q-prop, they use actor-critic to update parameter $w$ while here we use general control functional methods for variance reduction.

For the purpose of updating $\phi(s,a)$, we may consider minimizing 
\begin{align*}
\Var(\nabla_{\theta_\mu}J(\theta)) + \beta \Var(\nabla_{\theta_\Sigma}J(\theta))
\end{align*} 
w.r.t critic parameter $w$, where $\beta$ is a weight constant.



\subsection{TRPO with Stein control variate}
We first investigate applying Stein control variate to TRPO, and choose $Q_w(s_{t},a)|_{a= \mu_\theta(s_{t})}$ as Stein control variate.

For Gaussian policy, \eqref{equ:qprop} can be written in terms of both $\mu$ and $\Sigma$ as follows, 
\begin{align}
    \label{equ:mu}
    \nabla_{\theta_\mu} J(\theta ) & = \E_{\pi_{old}(a_t|s_t)}[ \frac{\pi_{\theta}(a_t|s_t)}{\pi_{old}(a_t|s_t)} [\nabla_\theta \log \pi_\theta(a_{t}|s_{t})(\hat{A}_{t} - Q_w(s_{t},a)|_{a= \mu_\theta(s_{t})}(a - \mu_\theta(s_{t}))  \\ \nonumber
    & + \nabla_{a}  Q_w(s_{t},a)|_{a= \mu_\theta(s_{t})} \nabla_\theta  \mu_\theta(s_{t})]],
\end{align}
\begin{align}
    \label{equ:sigma}
    \nabla_{\theta_\Sigma} J(\theta) = \E_{\pi_{old}(a_t|s_t)}[ \frac{\pi_{\theta}(a_t|s_t)}{\pi_{old}(a_t|s_t)} [ \nabla_\theta \log \pi_\theta(a_{t}|s_{t}) (\hat{A}_{t} - Q_w(s_{t},a)|_{a= \mu_\theta(s_{t})})(a - \mu_\theta(s_{t}))]],
\end{align}

Algorithm for TRPO with Stein control variate can be viewed in Algorithm \ref{alg:SteinTRPO}.


\begin{algorithm}[htbp]
  	\footnotesize
  	\caption{TRPO with Stein control variate. Modified from \citep{Schulman2015TrustRP}}
  	\label{alg:SteinTRPO}
  	\begin{algorithmic}[1] 
	\STATE Initialize $w$ for critic $Q_w$, $\theta$ for stochastic policy $\pi_\theta(\mu, \Sigma)$.
    \FOR {$i \in \{1, \cdots, N\}$}  
    \FOR {$ j \in \{1, \cdots, C\}$}
  	\STATE Optimizing parameters of $\phi_w(s,a)$ by minimizing $\Var(\nabla_\theta J(\theta))$ with ADAM.
  	\ENDFOR
  	\FOR {$ j \in \{1, \cdots, B\}$}
	\STATE Take a ADAM gradient step on $\theta_\mu$ using $\nabla_{\theta_\mu} J(\theta)$ in \eqref{equ:mu} .
	\STATE Take a ADAM gradient step on $\theta_\Sigma$ using $\nabla_{\theta_\Sigma} J(\theta)$ in \eqref{equ:sigma}.
	\ENDFOR
    \ENDFOR
  	\end{algorithmic}
\end{algorithm}

\subsection{Relation to Deterministic Policy}
Deterministic policy gradient \citep{Lillicrap2015ContinuousCW,silver2014deterministic} propose to use Ornstein–-Uhlenbeck process\citep{uhlenbeck1930theory} for exploring in deep deterministic policy. The Ornstein-–Uhlenbeck process models the velocity of a Brownian particle with friction,
which results in temporally correlated values centered around 0. 
If we choose $\phi =  Q(s,a)$ then our formula reduces to DDPG, we investigated this by fitting $\phi$ to advantage function in experiments.
Our general update rule,
$$
\nabla_\theta J(\theta) 
= \E[\nabla_\theta \log \pi(a|s) (Q^\pi(a,s)- \phi(a,s)] + \E[\nabla_\theta f(s, \xi) \nabla_a\phi(a,s)],
$$
can be viewed as a smoothing between the log-likelihood gradient estimator and a reparameterized gradient estimates. This connects to deterministic policy gradient \citep{Lillicrap2015ContinuousCW,silver2014deterministic} when $\phi = Q^\pi(a,s)$, arguably if $\phi$ approximate $Q^{\pi}(a,s)$ gradually along with training process proceeds, then our model can benefits from both exploration of stochastic policy and exploitation of deterministic policy at different training stage, Stein control variate can help reduce variance of Stochastic policy and reduce to deep deterministic policy when $\phi$ approximates $Q^\pi(s,a)$ well.

